vSPACE: Voting in a Scalable, Privacy-Aware and Confidential Election

The vSPACE experimental proof-of-concept (PoC) on the TrueElect[Anon][Creds] protocol presents a novel approach to secure, private, and scalable elections, extending the TrueElect and ElectAnon protocols with the integration of AnonCreds SSI (Self-Sovereign Identity). Such a protocol PoC is situated within a Zero-Trust Architecture (ZTA) and leverages confidential computing, continuous authentication, multi-party computation (MPC), and well-architected framework (WAF) principles to address the challenges of cybersecurity, privacy, and trust over IP (ToIP) protection. Employing a Kubernetes confidential cluster within an Enterprise-Scale Landing Zone (ESLZ), vSPACE integrates Distributed Ledger Technology (DLT) for immutable and certifiable audit trails. The Infrastructure as Code (IaC) model ensures rapid deployment, consistent management, and adherence to security standards, making vSPACE a future-proof solution for digital voting systems.

==> glos.tex <==
\newglossaryentry{GDPR}
{
name=GDPR (General Data Protection Regulation),
description={An EU regulation for data protection}
}


\newglossaryentry{IPFS}
{
name=IPFS (Interplanetary File System),
description={A distributed file system which uses a CID to link to a file}
}

\newglossaryentry{EMR}
{
name=EMR (Electronic Medical Record),
description={An electronic version of a patient health record}
}

\newglossaryentry{WHO}
{
name=WHO (World Health Organisation),
description={A United Nations organisation for public health on an international level}
}

\newglossaryentry{RTBF}
{
name=RTBF (Right-to-be-forgotten),
description={A core part of GPDR, and which defines that a citizen has the right to have their personal data removed from Internet searches}
}

\newglossaryentry{CDS}
{
name=CDS (Clinical Decision Support),
description={A health care system which allows improved clinical outcomes}
}

\newglossaryentry{KYC}
{
name=KYC (Know Your Customer),
description={A method which aims to gather key details about customers and that relate to their identity}
}

\newglossaryentry{HIPAA}
{
name=HIPAA (Health Insurance Portability and Accountability Act),
description={A US health regulation to protect health care information}
}

\newglossaryentry{Homomorphic Encryption}
{
name=HE (Homomorphic Encryption),
description={A method of public key encryption which allows data to be encrypted with a public key and then can be processed with the encrypted form. An associated private key will then decrypt the result}
}

\newglossaryentry{ZKP}
{
name=ZKP (Zero Knowledge Proof),
description={A method which protects the privacy of data, and where there is a proof of the knowledge of the data}
}

\newglossaryentry{RPM}
{
name=RPM (Remote Patient Monitoring,
description={A method of providing trusted monitoring of patients}
}
\newglossaryentry{Hyperledger}
{
name=Hyperledger (IBM Hyperledger,
description={An open-source permissioned ledger and supported by the Hyperledger Foundation.}
}

\newglossaryentry{Ethereum}
{
name=Ethereum,
description={A permissionless ledger that implements smart contracts}
}

\newglossaryentry{C3ISP}
{
name=C3ISP,
description={Cyber threat intelligence (CTI) has been proposed to achieve cyber threat information sharing between organisations}
}

\newglossaryentry{DIDs}
{
name=DIDs,
description={A decentralised Identifier}
}



\newglossaryentry{SSI}
{
name=SSI,
description={Self-sovereign identity}
}


\newglossaryentry{CTI}
{
name=CTI,
description={Cyber Threat Information}
}


\newglossaryentry{STIX}
{
name=STIX,
description={Structured Threat Information CybereXpression (STIX)}
}

\newglossaryentry{TAXII}
{
name=TAXII,
description={Trusted Automated eXchange of Indicator Information (TAXII)}
}

\newglossaryentry{ABE}
{
name=ABE,
description={Attributed-based encryption is a method that allows a policy to be defined for the encryption and decryption process, such as locking it down to specific time periods or for the location of the access.}
}

\newglossaryentry{FHE}
{
name=FHE,
description={Fully Homomorphic Encryption allows for every mathematical operation to be conducted on encrypted data. }
}















